Honeycomb-Surfels: Compact Hexagonal Primitives for Efficient Scene Rendering and Reconstruction

Novel view synthesis and 3D reconstruction have advanced rapidly with radiance fields and splatting, yet their memory and computational demands limit their use in resource-constrained settings. We introduce Hexels: novel planar hexagonal surface elements with a first-order spatial color field for efficient 3D scene and 2D image representation. Hexels exploit locally planar regions with smoothly varying appearance using fewer, larger primitives. Their hexagonal support provides an area- and boundary-efficient domain, while the local color field captures appearance variation within each primitive. Across 34 scenes, Hexels improve PSNR over memory-matched 2DGS by 4.53-7.38 dB across datasets while requiring lower training VRAM. We further ablate Hexels by showing that per primitive, Hexels outperform 2DGS by upto 4.74 dB while using lower training VRAM and having 2.31 times faster FPS. Even in unconstrained settings, Hexels offers complementary quality-memory trade-offs. For efficient 3D surface reconstruction, Hexels reduce error by 28.9% compared with memory-matched 2DGS across 15 DTU scans. On 6 Tanks and Temples surface scenes, Hexels achieves the highest mean F1 among compared methods (34.38%, versus 31.72% for 2DGS). We further also show that Hexels, as a general primitive, improves 2D image representation over Image-GS. Hexels push the Pareto frontier on the quality-efficiency trade-off of surface-aligned primitives.

==> Makefile <==
# make            -> build/sample.pdf with XeLaTeX (arXiv's engine)
# make lua        -> same with LuaLaTeX
# make compare    -> build/compare/sample-<scheme>.pdf for every font scheme
# make sheet      -> build/compare/sheet-page1.png and sheet-text.png contact sheets
# make arxiv      -> arxiv-upload/ ready to upload
# make MAIN=paper -> build another top-level file
MAIN    ?= main
SCHEMES ?= libron newsreader newsreader12 libertinus times stixtwo palatino charter utopia cm garamond kpfonts
OUT      = build

all: $(MAIN).tex
	latexmk -xelatex -outdir=$(OUT) $(MAIN).tex

lua: $(MAIN).tex
	latexmk -lualatex -outdir=$(OUT) $(MAIN).tex

watch:
	latexmk -xelatex -outdir=$(OUT) -pvc $(MAIN).tex

# One PDF per font scheme; the class option is injected with latexmk's
# -usepretex, so the .tex file itself is untouched.
compare: $(MAIN).tex
	mkdir -p $(OUT)/compare
	for s in $(SCHEMES); do \
	  latexmk -xelatex -outdir=$(OUT)/compare -jobname=$(MAIN)-$$s \
	    -usepretex="\\PassOptionsToClass{fonts=$$s}{myarxiv}" $(MAIN).tex || exit 1; \
	done
	@echo "PDFs in $(OUT)/compare/"

# Contact sheets (needs pdftoppm from poppler and magick from ImageMagick):
# page 1 of every scheme side by side, and a crop of page 3 (prose + math).
sheet: compare
	for s in $(SCHEMES); do \
	  pdftoppm -r 60 -png -f 1 -l 1 $(OUT)/compare/$(MAIN)-$$s.pdf $(OUT)/compare/p1-$$s; \
	  pdftoppm -r 150 -png -f 3 -l 3 $(OUT)/compare/$(MAIN)-$$s.pdf $(OUT)/compare/p3-$$s; \
	  magick $(OUT)/compare/p1-$$s-1.png -gravity North -background white -splice 0x28 \
	    -pointsize 20 -annotate +0+4 "$$s" $(OUT)/compare/p1-$$s.png; \
	  magick $(OUT)/compare/p3-$$s-3.png -crop 560x760+95+150 +repage -gravity North \
	    -background white -splice 0x30 -pointsize 22 -annotate +0+4 "$$s" $(OUT)/compare/p3-$$s.png; \
	done
	magick montage $(foreach s,$(SCHEMES),$(OUT)/compare/p1-$(s).png) -tile 5x -geometry +6+6 $(OUT)/compare/sheet-page1.png
	magick montage $(foreach s,$(SCHEMES),$(OUT)/compare/p3-$(s).png) -tile 5x -geometry +6+6 $(OUT)/compare/sheet-text.png
	rm -f $(OUT)/compare/p1-*.png $(OUT)/compare/p3-*.png
	@echo "Sheets: $(OUT)/compare/sheet-page1.png and $(OUT)/compare/sheet-text.png"

# Flat directory ready to upload to arXiv (fonts, figures, class, bst, bbl).
arxiv: all
	rm -rf arxiv-upload && mkdir -p arxiv-upload
	cp $(MAIN).tex myarxiv.cls papermacros.sty ACM-Reference-Format.bst ieeenat_fullname.bst $(OUT)/$(MAIN).bbl arxiv-upload/
	cp -r fonts figures arxiv-upload/
	@for f in preamble.tex main tables; do [ -e $$f ] && cp -r $$f arxiv-upload/; done; true
	@du -sh arxiv-upload | sed 's/^/bundle size (arXiv allows 50 MB): /'
	@echo "Upload the contents of arxiv-upload/ and choose XeLaTeX as the processor."

clean:
	latexmk -C -outdir=$(OUT) $(MAIN).tex
	rm -rf $(OUT) arxiv-upload

.PHONY: all lua watch compare sheet arxiv clean


==> figures/native_cell_boundary_export.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=\textwidth]{figures/assets/native_cell_boundary_export.pdf}
\caption{\textcolor{assistantorange}{\textbf{Native Hexel boundaries and polygonal Gaussian proxies.} (a) Different levels of a Gaussian weight field define different ellipses. (b) At $c=0.5$, six- and twelve-edge polygons approximate the selected ellipse (gray). (c) The six native Hexel vertices define its prescribed $d=0$ boundary exactly. This schematic concerns nominal cell geometry; both renderers use soft weights.}}
\label{fig:gaussian_polygonization}
\end{figure*}


==> main/10_applications.tex <==
% \section{Applications}
% \begin{figure*}[t]
%  \centering
%  \includegraphics[width=1\textwidth]{figures/skull_toy_combined.pdf}
%  \caption{\textbf{Direct surface extraction from Hexels}. Hexels provide an explicit surface representation that can be directly exported. The center column shows the wireframe (that is, the edges of the surface cell), and the right column visualizes the surface cells post-extraction.}
%  \label{fig:surface_export_references}
% \end{figure*}
% \subsection{Direct Surface-Cell Extraction}
% \label{app:surface_export}

% Hexels provide an explicit surface representation that can be exported
% directly after optimization from images. Unlike the depth-fusion pipeline
% used for mesh extraction in 2DGS~\cite{huang2024_2dgs}, this conversion
% requires no depth rendering, voxel grid, or Marching Cubes. The resulting
% surface cells can be used directly in object-centric applications such
% as 3D generation, segmentation, and representation learning.

% For each retained Hexel, we transform the six vertices of its canonical
% hexagon, defined by $d=0$, into world space using
% Eq.~\eqref{eq:plane-to-world}. Connecting consecutive vertices produces
% six edges and one polygonal face. Colors are obtained from the base
% RGB or evaluated from the spatial color field. Each cell remains
% associated with its parent Hexel, providing direct access to its geometry
% and appearance.

% The conversion requires $O(1)$ work per Hexel. The vertex positions and evaluated colors are differentiable with respect
% to the corresponding Hexel parameters. The exported cells can be optimized independently - opening up avenues for many downstream applications, both in 3D and 4D.
% Figure~\ref{fig:surface_export_references} shows the resulting wireframes and surface cells.

% \paragraph{Spatial color and extraction cost.}
% Figure~\ref{fig:surface_export_spatial} shows scan24 with the base-plus-gradient
% color field. Opacity filtering at 0.2 yields 20,021 exported cells and
% 120,126 sides. A separate projected-area filter of 4--2,000 pixels squared
% and visibility selection select 11,673 cells for the full-view wireframe
% before cropping. The warmed tensor conversion of all 20,021 exported cells
% takes 10.31\,ms median over 50 runs on one Intel Xeon E5-2637 v4 CPU thread,
% after ten warmups. Selection, checkpoint
% loading, hidden-line rendering, and serialization are excluded. This is
% an export measurement, not a novel-view FPS result or a comparison with
% mesh-extraction algorithms.

% \begin{figure*}[t]
%  \centering
%  \includegraphics[width=0.85\textwidth]{figures/assets/surface_cells_scan24.png}
%  \caption{A scan24 render and its directly exported colored cells.
%  The persistent color field is evaluated from the primitive coefficients,
%  without a learned texture atlas. This application uses an all-view model
%  and a visibility-filtered crop, separately from the NVS and fused-mesh
%  evaluations.\kk{combine with prev fig}}
%  \label{fig:surface_export_spatial}
% \end{figure*}

% \subsection{Deployment on Memory-Limited Devices}
% \label{app:mobile}

% Hexels require little model memory and training VRAM while retaining high
% reconstruction quality and fast rendering. These advantages are obtained
% in full precision, without texture atlases, neural decoders, pruning, or
% quantization. This makes Hexels well suited to reconstruction and rendering
% on memory-limited and edge hardware, and provides a basis for mobile
% deployment without changing the underlying primitive. Pruning and
% quantization could further reduce storage, but are not required for the
% efficiency demonstrated here.

% We have developed a Metal-based Hexel renderer and will release it alongside
% training code for memory-limited devices. The same hexagonal support and
% appearance model are retained, without converting the learned scene into
% a different representation for deployment. Hexels may have positive implications for on-device and privacy-conserving NVS and surface reconstruction. 

